AoI, Timely-Throughput, and Beyond: A Theory of Second-Order Wireless Network Optimization

This paper introduces a new theoretical framework for optimizing second-order behaviors of wireless networks. Unlike existing techniques for network utility maximization, which only consider first-order statistics, this framework models every random process by its mean and temporal variance. The inclusion of temporal variance makes this framework well-suited for modeling Markovian fading wireless channels and emerging network performance metrics such as age-of-information (AoI) and timely-throughput. Using this framework, we sharply characterize the second-order capacity region of wireless access networks. We also propose a simple scheduling policy and prove that it can achieve every interior point in the second-order capacity region. To demonstrate the utility of this framework, we apply it to an unsolved network optimization problem where some clients wish to minimize AoI while others wish to maximize timely-throughput. We show that this framework accurately characterizes AoI and timely-throughput. Moreover, it leads to a tractable scheduling policy that outperforms other existing work.

==> ge_model_case.tex <==
\section{A Special Case: Gilbert-Elliot Model} \label{sec:ge model}

Obtaining the explicit expressions for $\Bar{w}_i$ and $v_i$ is difficult for non-I.I.D channel, thus it is also difficult for $\mu_{\{S\}}$ and $\sigma_{\{S\}}^2$ while channels are independent with each other. 
In this paper, we study a simple Markovian model to obtain explicit expressions as a special case.
% special case
We consider the 2-state Markov approach as the Gilbert-Eliot model by Gilbert \cite{Gilbert1960GEmodel} and Elliot \cite{Elliot1963GEmodel} in Figure [xxx]. 
For each flow $i$, its connection process follows the Gilbert-Elliot model with a good (G) state and a bad (B) state, which represents the connection is ON and OFF respectively. 
The transition matrix $A$ is given as follow: 
\begin{align*}
    p_i &= Prob\{W_i(t) = 0|W_i(t-1) = 1\}\\
    r_i &= Prob\{W_i(t) = 1| W_i(t-1) = 0\}\\
    A_i &= \begin{pmatrix} 1-p_i & p_i \\ r_i & 1-r_i \end{pmatrix}.
\end{align*}  
Following the idea of Hablinger and Hohlfeld \cite{Gilbert1960GEmodel}, we can calculate the mean $T\Bar{w}_i$ and variance $Tv_i$ for any consecutive time slots $T$ via the generating functions. 
Specifically, we have:
\begin{align}
    T\Bar{w}_i &= (T+1)\frac{r_i}{p_i + r_i}\\
    Tv_i &= \frac{2Tr_i^2+Tp_ir_i}{(p_i+r_i)^2}  + \frac{2p_ir_i(1-p_i-r_i)}{(p_i+r_i)^3}T \notag \\ &\qquad- \frac{2p_ir_i((1-p_i-r_i)^2-(1-p_i-r_i)^{T+2})}{(p_i+r_i)^4}.
\end{align} The deviation can be found in Appendix []. 
